Drawing out of Distribution with Neuro-Symbolic Generative Models

Learning general-purpose representations from perceptual inputs is a hallmark of human intelligence. For example, people can write out numbers or characters, or even draw doodles, by characterizing these tasks as different instantiations of the same generic underlying process -- compositional arrangements of different forms of pen strokes. Crucially, learning to do one task, say writing, implies reasonable competence at another, say drawing, on account of this shared process. We present Drawing out of Distribution (DooD), a neuro-symbolic generative model of stroke-based drawing that can learn such general-purpose representations. In contrast to prior work, DooD operates directly on images, requires no supervision or expensive test-time inference, and performs unsupervised amortised inference with a symbolic stroke model that better enables both interpretability and generalization. We evaluate DooD on its ability to generalise across both data and tasks. We first perform zero-shot transfer from one dataset (e.g. MNIST) to another (e.g. Quickdraw), across five different datasets, and show that DooD clearly outperforms different baselines. An analysis of the learnt representations further highlights the benefits of adopting a symbolic stroke model. We then adopt a subset of the Omniglot challenge tasks, and evaluate its ability to generate new exemplars (both unconditionally and conditionally), and perform one-shot classification, showing that DooD matches the state of the art. Taken together, we demonstrate that DooD does indeed capture general-purpose representations across both data and task, and takes a further step towards building general and robust concept-learning systems.

==> old_text.tex <==
\section{Approach}\label{sec:approach}
\tnote{We should agree on which variables to use. Right now, we're using (A) $(\mathbf x, \mathbf z_{\text{what}}^{1:T}, \mathbf z_{\text{where}}^{1:T}, z_{\text{pres}}^{1:T}, n)$ in the text and (B) $(x_{1:T}, l_{1:T}, s_{1:T}, m_{1:T}, T)$ in the diagram.} \ynote{I would prefer (A), but also open for discussion)} 
\tnote{For (A), we should be consistent in using $T$ or $n$. Typically, I found it easy to read and write lowercase letters for an intermediate timestep and corresponding uppercase letters for the total number of timesteps since it is easier for the reader to remember what goes with what. E.g. $\sum_{t = 1}^T x_t$ or $\sum_{n = 1}^N x_n$ but not $\sum_{n = 1}^T x_n$ or $\sum_{i = 1}^N x_i$.} \ynote{Did I use $T$ at any place? I'm not finding any at the moment..}
\tnote{Should we bold or not? Bolding indicates that things are vectors but I have found that not to be that helpful to highlight.} 
\ynote{I like to have boldfaced letter to indicate vectors, but open for discussion.}\tnote{Using $z_{\text{what}}, z_{\text{where}}, z_{\text{pres}}$ vs $s, l, m$ is more intuitive for me and can resonate more with people familiar with AIR?}

\begin{figure}[t]
  \centering
  \input{figures/model}
  \caption{The \emph{generative model} produces an image of a handwritten character by sequentially sampling the stroke comprising the spline points ($s_t$) and the location ($l_t$).
  The rendered stroke $x_t$ is added to the previous intermediate rendering $x_{<t}$ to produce the current one $x_{\leq t}$.
  A binary on/off variable ($o_t$) determines whether to stop drawing.
  Differentiable rendering ($\delta R$) and differentiable affine transformation via Spatial Transformer Networks (STNs) \citep{jaderberg2015spatial} enables gradient-based learning.
  The \emph{recognition model} is conditioned on the image $x$ from which we subtract the intermediate rendering $x_{<t}$ to get the residual $\Delta x_t$ from which the model maps to the distributions over $l_t$ (where to draw next) and $o_t$ (whether to stop drawing).
  The distribution over the spline points $s_t$ is predicted from a crop of the residual, determined by the location $l_t$.
  Both models are autoregressive via two RNNs with hidden states $h_t^s$ and $h_t^l$.
  }
  \label{fig:model}
\end{figure}



To perform multiple tasks such as one-shot classification, imagining new examples, auto-completing example prompts (e.g. from half-written characters) with a single model, we build a flexible \emph{generative model} following carefully the causal and compositional data generating process. Specific to the stroke data domain, this means that all possible handwritten characters, sketches are constructed by sequentially select from a comparatively small set of strokes (such as sticks, humps, etc) and place on different regions of a canvas.
To learn such a model and make fast and reliable inference about the "underlying causes" (e.g. strokes) given high-dimensional perceptual data, we build a \emph{recognition model} closely mirroring the structure of the generative model.
These two components are built utilizing a hybrid of neural-symbolic techniques, borrowing their respective strengths. The two models learn jointly by bootstrapping each other in the spirit of the Helmholtz machine \cite{dayan1995helmholtz}, or the more recent variant, Variational Autoencoder \cite{kingma2013auto}.
This section introduces the generative and the recognition model, and their learning scheme.


\subsection{Generative Model}\label{sec:gen}
For observation $\x$ and latent variable $\z$, we have a two-level model of the form\footnote{This is resemblance on a high level to the generative model considered in AIR \cite{eslami2016attend} but distinct on lower levels}:

\begin{align}
    \ptheta(\x) = \sum_{n=1}^N\int \ptheta(\x, \z, n) d\z = \sum_{n=1}^N \ptheta(n) \int \ptheta^z(\z|n)\ptheta^x(\x|\z) d\z
    \label{eq:gen}
\end{align}
\tnote{Why is the sum finite and not infinite? Don't we want to be able to say that it's in principle infinite?} \ynote{re above, I think it helps to justify why we run the inference for a finite $N$ steps, instead of an infinite number of steps until all $\zpres=0$?}

In our domain, this can be interpreted as first sampling, from the \textbf{token model} $\ptheta(n)\ptheta^z(\z|n)$, the number of strokes $n$ from a suitable prior $\ptheta(n)$, and the symbolic latent stroke descriptors $\z=[\z^t]_{t=1}^n \sim \ptheta^z(\cdot|n)$.
Finally sample an image from the \textbf{image model}, $\x \sim \ptheta^x(\cdot|\z)$.

\paragraph{Image model.} Given a latent variable $\z$, the image model outputs an observation-dimensional distribution $\ptheta^x(\cdot|\z)$ parameterized by a deterministic, differentiable renderer $\rend(\z)$.
For an instance $\x\in\mathbb{R}^{H\times W}$  \tnote{Maybe $H \times W$ is more intuitive?} \ynote{Sure, $H,W$ is used in App. \ref{app:renderer} but we can swap them}, the distribution $\ptheta^x(\cdot|\z)$ is composed of $H\times W$ independent Laplace distributions with their means $\mu_{ij}$ equal $\rend(\z)_{ij}$ and scale being a global learnable parameter.

\paragraph{Token model.} The latent variables $[\z^t]_{t=1}^n$ with $\z^t=(\zwhere^t, \zwhat^t)$ are sampled sequentially with a factoring of $p(\z^1)\prod_{t=2}^n p(\z^t|\z^{<t})$. To make the conditioning more explicit, a canvas-so-far is created using the renderer from the image model, $\xbar^t=\rend(\z^{<t})$, and passed alone with the latent-so-far, $\z^{<t}$, when sampling $\z^t$, $\z^t \sim \ptheta(\cdot|\z^{<t}, \xbar^{t-1})$. This enables generation of highly structured data comparing to models with a stepwise independent prior, e.g. AIR \cite{eslami2016attend}.

\textbf{Prior and Sampling.} To aid the sequential generation and inference (discussed below) process, we parameterize $n$ using an equivalent representation of a variable length vector $\bzpres = [\zpres^t]_{t=0}^{n+1})$ using a unary code (a number $n$ is represented by $n$ ones followed by one zero). This empowers the model to decide either to continue or halt on each step $t$ based on the samples-so-far $(\zpres^{<t}, \z^{<t})$, and simplifies the auto-completion procedure from partially-finished samples, instead of committed to a fixed number at the outset. To simplify the notation, we use $\z^t$ to denote the concatenation of $\zpres^{t}$ and $\z^{t}$ defined above from now on.

Thence each latent $\z^t$ is a 3-tuple $\z^t=(\zpres^t, \zwhere^t, \zwhat^t)$ with decomposition Eq.~\ref{eq:latent_decom}. This describes the sampling process at each step: 
a)~if it is to continue generating strokes for at least one step (i.e. $\zpres^t=1$);
b)~what is the \emph{layout} (i.e. $\zwhere^t$) -- where it is going to place the next stroke -- e.g. with $\zwhere^t$ being a 4D vector specifying the x, y location, orientation and scale of a write-attention window $\xbarAtt^{t-1}$;
c)~what is the \emph{content} (i.e. $\zwhat^t$) -- which canonical stroke -- to draw down, by specifying a Bézier curve, e.g. the coordinates of $J=5$ control-points $[\p^t_j]_{j=1}^{J}$ of a degree-four Bézier curve in the attention window. These variables are all symbolic where each element has an assigned semantics, hence easily human interpretable, in contrast with distributed latents (e.g. the ones in AIR\cite{eslami2016attend}).

\begin{align}
    \ptheta(\z^t) = 
    \ptheta(\zpres^t, \zwhere^t, \zwhat^t) = 
    \ptheta(\zpres^t) \ptheta(\zwhere^t | \zpres^t) \ptheta(\zwhat^t | \zpres^t, \zwhere^t)
    \label{eq:latent_decom}
\end{align}
These variables are sampled from their respective distributions parameterized by neural nets, as described in Eq.\ref{eq:zpres_prior}-\ref{eq:zwhat_prior}. 
In detail, $\zpres^t$ is sampled from a Bernoulli distribution with parameterized by  $\iotapres(\xbar^{t-1})$, solely as a function of the drawing-so-far.
$\zwhere^t$ is sampled from a Gaussian Mixture Model (GMM) with $K$ components to capture the multimodel nature of handwritten character/drawings. Each component $k$'s mixing weight $\pi^t_{\mathrm{where},k}$, component location $\mu^t_{\mathrm{where},k}$, scale $\sigma^t_{\mathrm{where},k}$, and $x, y$ coordinate correlation $\rho^t_{\mathrm{where},k}$ is predicted by a neural net $\iotawhere(\hwhere^t)$, as in Eq. \ref{eq:zwhere_prior}, where $\hwhere^t$ is the hidden state of an RNN capturing all the information of about the latent-so-far (elaborated in Recurrence section).
$\zwhat^t$ is similarly sampled from a GMM. To capture the strong dependency between $\zwhere^t$ and $\zwhat^t$ in highly structured observations, $\zwhat^t$ is set to also explicitly depend on $\zwhere^t$ through both the $\zwhere^t$ values and the canvas-so-far $\xbar^{t-1}$ inside $\zwhere^t$ attention window, by employing a Spatial Transformer Network $\tau(\cdot,\cdot)$ \cite{jaderberg2015spatial}\footnote{Both $\zwhere^t$ and $\xbarAtt^{t-1}$ are inputted to $\iotawhat(\cdot)$ because $\zwhere$ disambiguates the attention output while $\xbarAtt$ makes the conditioning explicitly.}, i.e. $\xbarAtt^{t-1} = \tau(\zwhere^t, \xbar^{t-1})$. To combat with the complexity in the set of possible strokes with fine-grained and structural variations, we employ a GMM with $K$ components for \emph{each} control point $\p_j$, as well as correlations among $\p_j$'s $x, y$ coordinates, as in Eq.\ref{eq:zwhat_prior}.

\begin{align}
    \zpres^t\sim \mathrm{Bernoulli}(\cdot;p^t= \iotapres(\xbar^{t-1}))
    \label{eq:zpres_prior}\\
    \zwhere^t\sim \mathrm{GMM}(\cdot;[\pi^{t}_{\mathrm{where},k}, \mu^{t}_{\mathrm{where},k}, \sigma^{t}_{\mathrm{where},k}, \rho^t_{\mathrm{where},k}]_{k=1}^K = \iotawhere(\hwhere^{t}))
    \label{eq:zwhere_prior}\\
    \zwhat^t = [\p^t_j]_{j=1}^J, \p^t_j\sim \mathrm{GMM}(\cdot;[\pi^{t}_{\mathrm{what},jk}, \mu^{t}_{\mathrm{what},jk}, \sigma^{t}_{\mathrm{what},jk}, \rho^t_{\mathrm{what},jk}]_{k=1}^K)= \iotawhat([\hwhat^{t}; \zwhere^t; \xbarAtt^{t-1}])_j)
    \label{eq:zwhat_prior}
\end{align}


\textbf{Recurrence.} 
The hidden states $\h^t = (\hwhere^t, \hwhat^t)$ provide an efficient, distributed representation for conditioning the prior, at time $t$, on the latent-so-far $\z^{<t}$ with varying length $t$. They are updated through two Gated Recurrent Units (GRU) \cite{chung2014empirical} and shared with the inference network (discussed later), inspired by VRNN \cite{chung2015recurrent}. 
The canvas-so-far $\xbar^t$ is updated through gated elementwise addition (see App. \ref{app:renderer} for more detail).
The combined utilization of distributed ($\h^t$) and symbolic ($\xbar^t$) recurrent states demonstrated superior performance than using either of them alone.

\begin{align}
    \hwhere^t=\fwhere([\zwhere^{t-1};\xbar^{t-1}], \hwhere^{t-1})\\
    \hwhat^t=\fwhat([\zwhat^{t-1},;\xbar^{t-1}], \hwhat^{t-1})
    \label{eq:rnn}
\end{align}

Notably, AIR \cite{eslami2016attend} uses RNNs for the posterior inference, but with $\zwhat^{t-1}$ passed into $\fwhere$ instead of $\fwhat$. This together with the other explicit separation of \emph{content} from \emph{layout} bring forth a maximal transfer ability upon unseen data points.


\subsection{Inference}\label{sec:inf}
Despite the natural appeal of the generative model in Eq. \ref{eq:gen}, the posterior inference problem is usually intractable. Thence, we employ an amortized variational approximation $\qphi(\z|\x)$ of the true posterior $\ptheta(\z|\x)$, closely mirroring the structure of the generative model.
This leads to a sequential inference strategy of the form

\begin{align}
    \qphi(\z|\x) &= \qphi(\zpres^{n+1}=0|\z^{\leq n}, \x)
    \prod_{t=1}^{n} \qphi(\zwhere^t, \zwhat^t, \zpres^t = 1 | \z^{<t}, \x)
\end{align}

Given an observation $\x$, the network sequentially outputs parameters for the distribution of variable $\z^t$ conditioned on $\z^{<t}$ -- all the inferred variables from previous steps -- and the target $\x$.
The inference net runs for a maximum of $N$ steps; when $\zpres^t = 1$ it runs to predict parameters for at least one more step, when $\zpres^t = 0$ the run terminates for this particular observation $\x$.

The conditioning on the latent-so-far is achieved through the shared RNN with the prior, as introduced in Eq. \ref{eq:rnn}.
We further leverage the principle of analysis-by-synthesis by taking a residual image $\deltax^t:=\x-\xbar^t$ as input of the inference net, facilitating the network to focus on the unexplained strokes.

Specifically, the posterior distribution of $\zwhere$ and $\zwhat$ has the same form as in the prior except with a single mixture component:

\begin{align}
    \zwhere^t \sim \mathcal{N}(\cdot;(\mu^{t}_{\mathrm{where}}, \sigma^{t}_{\mathrm{where}})= \lambdawhere(\hwhere^{t}, \deltax^{t}, \x))
    \\
    \zwhat^t = [\p^t_j]_{j=1}^J, \p^t_j \sim \mathcal{N}(\cdot;(\mu^{t}_{\mathrm{what},j}, \sigma^{t}_{\mathrm{what},j}, \rho^t_{\mathrm{what},j})= \lambdawhat(\hwhat^{t}, \deltaxAtt^{t-1}, 
    \xAtt^t)_j)
    \\
    \zpres^t \sim \mathrm{Bernoulli}(p^t),~\mathrm{where}~p^t= \lambdapres(\deltax^{t-1}, \rho_{\mathrm{rsd}})\\
\end{align}

Symmetrical to the use of write attention in the prior, a read attention $\tau(\cdot, \cdot)$ is used by the model to focus the region in the residual/target to be explained next, $\deltaxAtt^{t-1}=\tau(\zwhere^t,\deltax^{t-1}), \xAtt^{t-1}=\tau(\zwhere^t,\x)$, while framing the target stroke into a canonical position, reducing the workload of $\lambdawhat$ hence facilitate generalization.

Notably, for the posterior of $\zpres^t$, instead of keeping it symmetrical to the prior, we pass it the residual pixel ratio $\rho_{\mathrm{rsd}}:=\frac{\sum_{ij}\deltax_{ij}}{\sum_{ij}\x_{ij}}$ -- the quotient of the sum of the pixel intensities of the residual and that of the target. This means that whether the inference continues is mainly dependent on the amount of pixels to be explained. This allows strong and robust generalization ability over reasoning about the appropriate number of strokes to use compared to AIR \cite{eslami2016attend}, as we show in \ref{sec:exp}.


\subsection{Learning}\label{sec:learning}
One way of learning the parameters of the model $\theta$ and the inference network $\phi$ is by jointly maximizing the lower bound of the marginal likelihood of an image $\x$:

\begin{align*}
    \log \ptheta(\x)
    &= \log\int d\z \ptheta(\x, \z)
    = \log\int d\z \sum_n \qphi(\z|\x) \frac{\ptheta(\x, \z, n)}{\qphi(\z|\x)}\\
    &= \log\Eqphi[ \frac{\ptheta(\x, \z)}{\qphi(\z|\x)} ]
    \geq \Eqphi[\log\frac{ \ptheta(\x, \z)} {\qphi(\z | \x)}]\\
    &= \Eqphi[\log\ptheta(\z)] + \Eqphi[\log\ptheta(\x|\z)] - \Eqphi[\log\qphi(\z|\x)] =: \L(\theta, \phi)
\end{align*}

A Monte Carlo gradient estimator for $\pdv{}{\theta}\L$ is relatively easy to compute by drawing $(\z) \sim \qphi(\cdot|\x)$ and compute $ \pdv{}{\theta}  \log p_\theta(\x, \z)$ as the model is differentiable to its parameters.

Estimating the gradient for $\pdv{}{\phi}\L$ is more involved as the parameters $\phi$ are also used when drawing samples $\qphi$ but not in computing $\log \ptheta(\x, \z)$. To address this, for each step $t$, denote $\omega^t$ all the parameters of the distribution on variables $(\z^t)$, we parameterize the dependency of this distribution on $(\z^{<t}, \x)$ using a recurrent function $R_\phi$ implemented using a recurrent neural network. At each step $t$, $(\omega^t, \h^t)=R_\phi(\x, \xbar^{t-1}, \h^{t-1})$, with canvas $\xbar$ and hidden variables $\h$. The full gradient can therefore be obtained via chain rule: $\pdv{\L}{\phi}=\sum_t\pdv{\L}{\omega^t}\pdv{\omega^t}{\phi}$.
Let $z^t$ be an arbitrary variable in $(\zwhere^t, \zwhat^t, \zpres^t)$ and define $\ll := \log \frac{\ptheta(\x, \z)}{\qphi(\z|\x)}$, we can write the loss as $\L(\theta,\phi) = \Eqphi[\ll]$, how to proceed with computing $\pdv{\L}{\omega^t}$ depends on whether $z^t$ is discrete or continuous.

\textbf{Continuous.} For continuous random variable $z^t$, we can use the reparametrization trick to back-propagate through $z^t$ \cite{kingma2013auto, schulman2015gradient}. The trick suggest that for many continuous random variables, drawing a sample $z^t$ from the distribution parameterized by $\omega^t$ yields an equivalent result as taking the output of a deterministic function inputting some random noise variable $\xi$ and parameter $\omega^t$, $z^t = d(\xi, \omega^t)$ where $\xi$ is sampled from some fixed noise distribution $p(\xi)$. This results in the estimator: $\pdv{\L}{\omega^t} \approx \pdv{\ll}{z^t} \pdv{d}{\omega^t}$.

\textbf{Discrete.} For discrete variable such as $\zpres^t$, the reparametrization trick can't be applied. Instead, we resort to the REINFORCE estimator \cite{mnih2014neural, schulman2015gradient}, with a Monte Carlo estimate of the gradient: $\pdv{\L}{\omega^t} \approx \pdv{\log\qphi(\z|\x)}{\omega^t} \ll$.

This can be derived as follows (denote $\ll$ by $\ell(\z)$ and $\qphi(\z|\x)$ by $\qphi(\z)$ to reduce cluster):

\begin{align*}
    \pdv{\L}{\omega^t}
    &= \pdv{}{\omega^t} \int  \qphi(\z) \ell(\z) d\z \\
    &= \int(\pdv{}{\omega^t}\log \qphi(\z))  \qphi(\z) \ell(\z) d\z \\
    &= \mathbb{E}_{\qphi(\z)} [\pdv{}{\omega^t} \log \qphi(\z) \ell(\z)] \\
    &\approx \pdv{\log\qphi(\z)}{\omega^i} \ell(\z)
\end{align*}

This basic form usually results in a high variance, and we can significantly reduce it by using only local learning signals and a structured neural baseline\cite{mnih2014neural}.  The former suggests that we can remove the terms in $\ell(\z)$ that doesn't depend on $\omega^t$ without affecting the result, this allows us to substitute $\ell(\z)$ with $\ell^t(\z) := \log\ptheta(\x|\z) \ptheta(\z^{t:N}) / \qphi({\z^{t:N}})$ such that it only uses learning signals dependent on $\omega^t$.  Further, the latter suggests adding a negative $b(\z^{<t},\x)$ term--which takes in the previous variables $\z^{<t}$ detached from the gradient graph and $\x$--next to $\ell^t(\cdot)$. It is trained by minimizing the mean squared error between $\ell^t(\cdot)$ and $b(\z^{<t},\x)$, $\L_b := \mathbb{E}_{\qphi}[(\ell^t(\z)-b(\z^{<t},\x))^2]$. This yields an improved, final estimator used in learning $\pdv{\L}{\omega^t}\approx\pdv{\qphi(z^t)}{\omega^t} \left( \ell^t(\z) - b(z^{<t}, \x) \right)$.  The final loss function can be written as $\hat\L = \L + \L_b$.



\section{Experiments (OLD)}\label{sec:exp}

\snote{Include a section about ``this is all the tricks we had to do''.}


We evaluate our model along two diagonal axes -- broad and deep generalization.
In the first, we evaluate the model's ability to generalize across a broad range of dataset distributions.
We train an instance of the model described in \cref{sec:method} on each of the five stroke-based datasets with 50$\times$50 resolution images. They include MNIST of handwritten digits \cite{lecun1998mnist}, EMNIST of handwritten character digits \citep{cohen2017emnist}, KMNIST of deformed Japanese characters \citep{clanuwat2018deep}, Omniglot handwritten characters from 50 alphabets \citep{lake2015human}, and Quickdraw of hand drawings \citep{ha2017neural} (details in \cref{app:dataset}). 
Our model demonstrates strong cross-domain generalization quantitatively and qualitatively through marginal likelihood evaluation, inference inspection in all datasets, and latent representation classification in all but Omniglot dataset (due to its disjoint dataset structure).
Deep generalization is demonstrated by the wide range of tasks that a model supports through its rich representation.
Our model is further evaluated on three Omniglot challenge tasks  -- unconditional generation, character-conditional generation and one-shot classification \citep{lake2015human} -- as well as prior sampling in the other 4 datasets.

In all tasks, the models are trained with a maximum number of $N=6$ strokes,  4-dim $\zwhere^t$ describing the positions, scale, rotation of the attention window and 10-dim $\zwhat^t$ specifying the coordinates of 5 control-points. Convolutional neural nets (CNN), $\upsilon(\cdot)$, are used as feature extractors for images (one for canvas-so-far, attention window, target, another for residual and its counterparts).
In addition, a small MLP, taking the same input as $\lambdawhere()$, is used to predict the 3 renderer parameters at each step $t$, roughly controlling the stroke thickness and brightness, which are not modelled as random variables. More details of the renderer and training scheme is discussed App.~\cref{app:renderer} and \cref{app:training} respectively.

\subsection{Broad Generalization}
\subsubsection{Zero-shot reconstruction}
With a recognition network learned for posterior inference from one data distribution (e.g. MNIST), one desideratum is it would generalize well to other data distributions of the same concept class (e.g. Omniglot) -- i.e. to make fast yet accurate posterior inference and subsequently reconstructions. In this experiment, we qualitatively inspect the posterior inference quality of the model conditioning on observations with varying degrees of composition-complexity deviations from the training dataset. 
We then quantitatively evaluate it by computing the marginal likelihood under the principle of "conservation of belief", as approximated by the importance weighted autoencoder metric \cite{burda2015importance}.

We compare our model with a state-of-the-art sequential generative model DAIR, a variant of AIR with stronger generalization ability\citep{eslami2016attend} and a range of lesion models, highlighting key design choices. 
We use a reproduced implementation of DAIR (as the original implementation is not publicly available) with the same neural net capacity as our model (which has improved performance over the original implementation; for details of the neural net configuration, see App~\cref{app:nn_config}).
For ablations study, we evaluated the model without the 3 key ingredients separately: 1)~learnable sequential prior; 2)~Bézier curve decoder; 3)~guided-execution. 
For 1), the prior MLPs taking in the recurrent states are replaced with AIR-style, fixed prior distributions. 
In 2), the analytical Bézier-curve decoder is replaced with a neural net, the exact one as used in our DAIR implementation. It's important to note that only precisely the decoder function -- inputting $\zwhat$, outputting unnormalized pixel-values -- has been substituted, i.e. the constraints on the posterior parameters, normalization procedure, image distribution, etc are kept the same as the full model. 
In 3), all residual $\deltax$ or canvas-so-far $\xbar$ variables used in running the model have been removed from the function-input list.

To begin with, we train all models on visually the simplest dataset, MNIST, and inspect their zero-shot generation ability by looking at their step-by-step inference quality on all test datasets, as shown in \cref{fig:mnist_generalization}. We then investigate in the overall zero-shot generalization of varying difficulties by running all the train/test-dataset combination, with results shown in the confusion matrix in \cref{fig:all_cross_ds_eval}.

\begin{figure}[h!]
\captionsetup[subfigure]{labelformat=empty} %
\centering
\input{figures/mnist_transfer_cumulative_recon}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/mnist_trans_recon/z_pr_generalize_Full.pdf}
    \caption*{Our model}
    \label{fig:z_pres_generalization_full}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/mnist_trans_recon/z_pr_generalize_DAIR.pdf}
    \caption*{DAIR}
    \label{fig:z_pres_generalization_dair}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/mnist_trans_recon/z_pr_generalize_AIR.pdf}
    \caption*{AIR}
    \label{fig:z_pres_generalization_air}
\end{subfigure}
\caption{\ynote{Removed SSP-Sequential Prior} Our model generalizes better than DAIR.
(a) Our model trained on MNIST reconstructs characters from all other four datasets while the baseline DAIR model's reconstructions are often inaccurate, blurry or incomplete.
Explicit splines or intermediate renderings are responsible for this generalization which degrades when using our model without either of these components.
(b) Our model learns to use more strokes than it was trained on, unlike DAIR.}
\label{fig:mnist_generalization}
\end{figure}


\begin{figure}[]
\centering
\includegraphics[width=1\linewidth]{figures/cross_dataset_mll.png}
\caption{\ynote{Will use a shared color bar between 2 confusion matrixes} When training on one ``source'' dataset and testing on another ``target'' dataset, our model has a higher log likelihood and better reconstructions than DAIR. Training on Omniglot as a source dataset leads to the worst transfer (the Omniglot row is the darkest) as the stroke thickness is mismatched.}
\label{fig:all_cross_ds_eval}
\end{figure}

As demonstrated in \cref{fig:mnist_generalization}, our model is able to generalize strongly with respect to the following 3 aspects. 
1.~Most notably, we observe that our model makes overall more accurate reconstructions than DAIR across all target distributions.
This highlights the utility of, especially when limited data is available, constraining the model and leveraging the causal knowledge such that it still learns the compositional structure of the observation, such as in our case learning the simple images are composed of strokes, as opposed to DAIR trying to explain the whole image with 1 or 2 steps that ultimately led to poor out-of-distribution generalization.
2.~Despite that SSP isn't pixel-perfect in zero-shot reconstruction, which can be largely attributed to the $\zwhat$ component of the recognition model, we see that the $\zpres$ component has generalized incredibly well: despite using mostly 2 strokes on the source dataset MNIST and is limited to the maximum rollout number of $N=6$ during training, it is able to make use of a significant larger amount of strokes when needed during testing. 
In particular, as shown in \cref{fig:z_pres_generalization_full} histograms, when allowed to run for $N=10$ steps in evaluation, SSP is able to make full use of the given max flexibly and controllably; using mostly 10 strokes in QuickDraw to compensate for the deficiency in the $\zwhat$ module, while still using mostly 2 and 4 strokes in MNIST and Omniglot respectively. This is in stark contrast with the inflexibility of DAIR, 
which stresses the importance of having a modular design (not having an $\zpres$ RNN) and providing it with the appropriate inputs (i.e. residual and residual-pixel count but not the canvas-so-far nor the target).
3.~Qualitatively, SSP outperforms DAIR in marginal likelihood across all test data distributions, confirming the qualitative results.

Compare to Abl1 which doesn't use a learnable, sequential prior, we observe Abl1 has only slight worse in reconstruction quality as also indicated by the minor decrease in marginal likelihood. This isn't surprising, as the sequential prior is mainly responsible for a more realistic unconditional sampling (as shown in \cref{sec:uncon_gen}) and bootstrapping the joint learning between the posterior and the prior during training.
Compare to Abl3 which doesn't use intermediate rendering, not only is it struggling when transfer to especially more complex dataset, e.g. Omniglot or QuickDraw,  due to a lack of intermediate feedbacks, it also has degenerated control over the number of strokes employed, notably, taking 6 strokes to draw a character "1", highlighting again the significance of exploiting intermediate feedback.

\ynote{to do: cross dataset experiment analysis}

\subsubsection{Latent Classification and Visualization}
As motivated by \citet{eslami2016attend}, structured models are also useful as their inference can provide useful representation for downstream tasks.
In this regard, our symbolic latent approach already has the advantage of being readily human-interpretable and easier to work with interactively (e.g. as shown in \cref{sec:partial_completion}, partial-completion). Here, we investigate the utility of the inferred latents towards a downstream machine learning task -- classification.

In this experiment, the models learned on each dataset (from the previous section) are used to parse the images in all datasets. The inferred $[\zwhere^t, \zwhat^t]$ variables are masked with $[\zpres^t]$ then concatenated into a single vector before feeding into a multi-class logistic regression classifier, which is trained on the cross entropy loss until convergence.
We further inspect the learned latent space by visualizing the TSNE embedding of the $\zwhat$ latents infer from MNIST images (by the MNIST-trained model) in \cref{fig:tsne}.

The classification results of SSP vs. DAIR is shown in \cref{fig:lv_clf_vis} confusion matrices, showing an overall stronger performance of SSP over DAIR.

\begin{figure}[h!]
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/cross_trans_quantitative/cross_dataset_clf_heatmap_5e5_full.pdf}
  \caption{}
  \label{fig:ours_cross_clf}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/cross_trans_quantitative/cross_dataset_clf_heatmap_5e5_dair.pdf}
  \caption{}
  \label{fig:dair_cross_clf}
\end{subfigure}\\
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/tsne_Full_kmeans8_sc0.21-tab.pdf}
  \caption{}
  \label{fig:tsne}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/tsne_DAIR_kmeans8_sc.11-tab.pdf}
  \caption{}
  \label{fig:tsne}
\end{subfigure}
\caption{Training a linear classifier on top of the inferred latent variables has a higher accuracy for our model than DAIR. A TSNE embedding of inferred latent variables from our model results in interpretable clusters of strokes. The embeddings' colour is obtained from a K-Means clustering on the $\zwhat$s directly, with $K=8$. SSP's cluster scored a Silhouette Coefficient (sc) of 0.21, DAIR 0.11.}
\label{fig:lv_clf_vis}
\end{figure}

While our model is already more human-interpretable with its disentangled symbolic latent representation, experiments show that such representation is also more useful for machines in classification. 
With the TSNE plot showing the learned "stroke bank" of our model, it prospects the potential for strong performance even when using simpler, more human-interpretable classifiers, e.g. a decision tree based on the set of prototypical strokes used in parsing each image.


\subsection{Deep Generalization}\label{sec:deep_gen}
Akin to human learning, generative models, especially the ones with symbolic latent representation like SSP, are useful in the multitude of tasks they support with a single learned representation, 
such as creatively imaging new exemplars when given a reference image, generating new concepts without explicitly referring to any examples, and classifying observations under a single model. We assess our generative in the above 3 tasks respectively. In the context of the Omniglot dataset, these correspond to three of the Omniglot challenge tasks \citep{lake2015human}.

To naturally fit our model into the Bayesian formulation of especially the latter 2 tasks, we make a straightforward and natural modification to our \textbf{token model}. With the learned generative and recognition model, we can regard the learned \textbf{token model} $p(\z)$ as a higher-order \textbf{type model} $p(\psi)$, incorporate a new token model $p(\z|\psi)$, and consider the learned variational posterior $q(\z|\x)$ to be directly on the type variable $\psi$, i.e. $q(\psi|\x)$.  
With this setup, the token model $p(\z|\psi)$ captures the plausible structural variabilities of various instances of a character (e.g. affine transformations, motor noises). This can either be learned or set by heuristics. In our experiment, we leverage a simple uniform distribution over a range of affine transformations and a spherical normal distribution for motor-noise.
Note that the flexibility of doing this is thanks to the symbolic latent representation that our model has, while models with distributed latent representations lack.

\subsubsection{Unconditional Generation}\label{sec:uncon_gen}
We examine the quality of samples drawn from the learned generative model. On one aspect, if the model can generate dataset-representative images, we can verify that the model is learning to learn, and the task of learning the variational posterior would be greatly simplified. On the other, it can act as a source of generating labelled synthetic dataset.
Taking the generative model from the joint training above, we feed the generative model the same initial recurrent states (canvas-so-far and RNN hidden states) as during training and draw the prior samples onto the canvas-so-far before passing them into the model again.
\cref{fig:uncon_gen} shows some generation results with models learned on each dataset.

The samples show that SSP generates highly-structured data-distribution representative images, emphasizing the advantage of having a learnable, sequential prior.

\ynote{Will add a part reporting the FID score if time allows}

\begin{figure}[h!]
  \setlength\tabcolsep{0.08cm}
  \centering
  \begin{tabularx}{\linewidth}{X|X|X|X|X}
  MNIST & EMNIST & KMNIST & QuickDraw & Omniglot \\
  \hline
  \adjincludegraphics[width=.2\textwidth, trim={0 0 {.75\width} 0},clip]{figures/uncon_generation/uncon_gen_mn.pdf} &
  \adjincludegraphics[width=.2\textwidth, trim={0 0 {.75\width} 0},clip]{figures/uncon_generation/uncon_gen_em.pdf} &
  \adjincludegraphics[width=.2\textwidth, trim={0 0 {.75\width} 0},clip]{figures/uncon_generation/uncon_gen_km.pdf} &
  \adjincludegraphics[width=.2\textwidth, trim={0 0 {.75\width} 0},clip]{figures/uncon_generation/uncon_gen_qd.pdf} &
  \adjincludegraphics[width=.2\textwidth, trim={0 0 {.75\width} 0},clip]{figures/uncon_generation/uncon_gen_om.pdf}\\
  \end{tabularx}
  \caption{\ynote{Will invert the color and update before end of 14th; will try to add GNS comparison} Our model generates high quality unconditional character samples which are visually indistinguishable from the real characters as it successfully captures the stroke shape and the stroke structure.}
  \label{fig:uncon_gen}
\end{figure}

\subsubsection{Partial Completion}\label{sec:partial_completion}
Provided images with "partial-completed" sketches/characters, SSP can imagine likely ways that the images can be more completed.

To perform this task, SSP requires us to provide both the canvas-so-far and the RNN recurrent states.
While the partial-completed images can be readily regarded as canvas-so-far, we also need to address the need for the RNN recurrent states.
Owing to the sharing of the RNNs between the generation and recognition model, we can use the recognition model to provide the hidden-states as it parse through the partial images. This is in contrast to having to provide some random recurrent states to the RNNs, which we've found to degrade the completion quality.

\begin{figure}[h!]
\setlength\tabcolsep{0.08cm}
\captionsetup[subfigure]{labelformat=empty} %
  \centering
  \begin{tabularx}{\linewidth}{ccccc}
  MNIST & EMNIST & KMNIST & QuickDraw & Omniglot\\
  \adjincludegraphics[width=.19\linewidth, trim={0 {.874\height} 0 0},clip]{figures/partial_completion/par_com_mn.pdf} &
  \adjincludegraphics[width=.19\linewidth, trim={0 {.874\height} 0 0},clip]{figures/partial_completion/par_com_em.pdf} &
  \adjincludegraphics[width=.19\linewidth, trim={0 {.874\height} 0 0},clip]{figures/partial_completion/par_com_km.pdf} &
  \adjincludegraphics[width=.19\linewidth, trim={0 {.874\height} 0 0},clip]{figures/partial_completion/par_com_qd.pdf} &
  \adjincludegraphics[width=.19\linewidth, trim={0 {.874\height} 0 0},clip]{figures/partial_completion/par_com_om.pdf} \\
  \end{tabularx}
  \caption{Given a partially drawn character, our model can generate a realistic distribution over its completions by sampling from the generative model conditioned on the image of the partial character.}
  \label{fig:uncon_gen}
\end{figure}

\subsubsection{Character-Conditioned Generation}
Upon seeing merely one example of a concept such as a handwritten character, humans can generate new exemplars of the same concept with significant variations while maintaining salient structural properties. This demonstrates the rich and flexible representation that human learns from few examples.

SSP can perform this task in a natural Bayesian setting when equipped with the plug-and-play token model $p(\z|\psi)$, as described at the beginning of \cref{sec:deep_gen}. We use $q(\psi|\x)$ to infer the type variable when given an observation $\x$, and plausible token samples can be drawn from the token model then rendered using the image model.

The results of some Omniglot-character conditioned generations are shown in \cref{fig:char_con_gen}, capturing very human-like variabilities.


\begin{figure}[h!]
  \captionsetup[subfigure]{labelformat=empty} %
  \centering
  \begin{tabularx}{\linewidth}{c}

  \adjincludegraphics[width=.97\linewidth, trim={0 0 0 {.91\height}},clip]{figures/char_con_gen.pdf} \\
\hline

  \adjincludegraphics[width=.97\linewidth, trim={0 {.09\height} 0 0 },clip]{figures/char_con_gen.pdf} \\
  \end{tabularx}
  \caption{Given a target image of a handwritten Omniglot character (above the horizontal line), our model produces realistic new exemplars by inferring an explicit stroke-based representation.}
  \label{fig:char_con_gen}
\end{figure}

\subsubsection{One-shot Classification}
Given just a couple of examples of a few characters from an alphabet, humans can easily categorize which two are instances of the same character accurately. Discriminative model are mostly designed and trained to perform only this one-shot classification task\citep{vinyals2016matching, finn2017model, snell2017prototypical}, whilst most successful generative approaches\citep{feinman2020learning, hewitt2018variational, lake2015human} make use of extra supervisions, e.g. the structural knowledge of the dataset, data augmentation during training.
We aim to demonstrate that competitive performance can be achieved with our unsupervised generative model, without using data augmentation, in the original, most challenging (i.e. within-alphabet rather than between-alphabet) formulation of the Omniglot one-shot classification task \citet{lake2015human}. In particular, our model wasn't trained as a hierarchical model, as some other generative models are \citep{feinman2020learning, hewitt2018variational}.

SSP performs this task as follows. When given a single support image $\xc$ from each class $c=[1,C]$, and a query image $\xT$, it classifies which class $\xT$ it belongs to by computing the Bayesian score $p(\xT|\xc)$ and predicting the $c$ with the highest score. The score is computed by:

\begin{align}
    p(\xT|\xc) 
    &= \int p(\xT, \zT, \psic | \xc) d(\zT, \psic)\\
    &\approx \int p(\xT|\zT) p(\zT|\psic) p(\psic|\xc) d(\zT, \psic)\\
    &\approx \sum_{k=1}^K \pi_k\max_{\zT} p(\xT|\zT) p(\zT|\psic_k)\\ &~\text{where}~\psic_k \sim p(\psic|\xc), \pi_k\propto\tilde{\pi}_k=p(\psic_k, \xc)~\text{and}~\sum_{k=1}^K \pi_k = 1\\
\end{align}
where $p(\zT|\psic)$ is the plug-and-play token model (as introduced in the beginning of \cref{sec:deep_gen}) taking the potential affine transformation, motor noise into consideration.

The original task includes 20 episodes, each a 1-shot 20-way classification problem with samples from a distinct alphabet unseen during training. The preliminary results are shown in Table.~\cref{tab:one_shot_clf}.

\include{tables/one_shot_clf_result_table}

\section{Related work}
Our framework is an instance in the class of unsupervised, sequential, neural-symbolic generative models that brings together the principles of compositionality, causality and learning-to-learn. And our model focuses on its application to stroke-based data.

The major component in our framework is a generative model, a model capable of generating observation data $x$, e.g. images of handwritten characters. And it's closely related to the Variational Inference (VI) \cite{kingma2013auto} and Autoregressive (AR) \cite{reed2017parallel} approach to deep generative modelling, in contrast to the Generative Adversarial Networks (GANs) approach.

Our generative model samples data sequentially, object-by-object, more specifically in our case, stroke-by-stroke, guided by the principle of compositionality. In this sense, the generative model and its accompanying inference network belongs to one of the two main approaches to object-centric representation learning -- the bounding-box approach \cite{eslami2016attend, rezende2016one, gregor2015draw}; while the other being the scene-mixture approach \cite{burgess2019monet, greff2019multi}, which attempts to generate samples as mixtures of image layers ideally one object per layer.
Distinct from most neural approach with mainly distributed latent representation and neural decoder, we have a neural-symbolic generative model, where purely symbolic latent variables $z$ are sampled from a deep autoregressive prior \cite{chung2015recurrent} and processed by a symbolic, differentiable rasterizer, such as \cite{li2020differentiable} to produce the observation distribution $x|z$, following the principal of causality.
In this spirit, the generative model is analogous to that in GNS \cite{feinman2020learning}, but different in that we use an unsupervised, variational inference approach using solely the raw image data, whereas GNS uses stroke-level supervision (the location and segmentations of character strokes). \cite{ha2017neural, chung2015recurrent} also employs the variation inference approach to stroke data, but again, trains with stroke-level supervision.

The structured sequential inference (recognition) network is an instance of amortized inference, in contrast to MCMC methods. The sequential process reflects the principle of analysis-by-synthesis, where the observation is continually integrated with the intermediate representation of it to guide the inference \cite{yuille2006vision}. The recognition net is applied to infer both continuous and discrete random variables, and is learned through the pathwise derivative (reparametrization) estimator \cite{kingma2013auto, rezende2014stochastic} and score function (REINFORCE) estimator \cite{mnih2014neural}, for the two variables types respectively. On a high level, the recognition model is similar to that of the other sequential VI models, but with key design changes such as the use of intermediate canvas, residual image, separation between layout and content variables to facilitate generalization.

The generative and inference model are optimized jointly under the variational free energy objective, facilitating a form of learning-to-learn \cite{hospedales2020meta}. Closely related to this objective, one could optimize the criterion with the reverse KL term, yielding the wake-sleep algorithm \cite{hinton1995wake}.

This work is also an example of program induction \cite{ellis2020dreamcoder, balog2016deepcoder, devlin2017robustfill, liang2010learning, lake2015human} with a library of learned graphics programs with minimal syntax.


==> tables/one_shot_clf_result_table.tex <==
\begin{table}
  \caption{Our model achieves competitive one-shot classification accuracies.}
  \label{tab:one_shot_clf}
  \centering
  \begin{tabular}{ll}
    \toprule
    Model    & Accuracy \\
    \midrule
    Ours & 73.5\%    \\
    VHE\cite{hewitt2018variational}  & 81.3\%  \\
    GNS\cite{feinman2020learning}  & 94.3\%  \\
    BPL\cite{lake2015human} & 96.7\% \\
    \bottomrule
  \end{tabular}
\end{table}
